CANF-VC: Conditional Augmented Normalizing Flows for Video Compression

This paper presents an end-to-end learning-based video compression system, termed CANF-VC, based on conditional augmented normalizing flows (CANF). Most learned video compression systems adopt the same hybrid-based coding architecture as the traditional codecs. Recent research on conditional coding has shown the sub-optimality of the hybrid-based coding and opens up opportunities for deep generative models to take a key role in creating new coding frameworks. CANF-VC represents a new attempt that leverages the conditional ANF to learn a video generative model for conditional inter-frame coding. We choose ANF because it is a special type of generative model, which includes variational autoencoder as a special case and is able to achieve better expressiveness. CANF-VC also extends the idea of conditional coding to motion coding, forming a purely conditional coding framework. Extensive experimental results on commonly used datasets confirm the superiority of CANF-VC to the state-of-the-art methods. The source code of CANF-VC is available at https://github.com/NYCU-MAPL/CANF-VC.

==> chapter/2-1_compare_table.tex <==
\begin{table*}[t]
\centering%
\caption{.}
\label{tab:exp_BD_PSNR}
\setlength{\tabcolsep}{3mm}{
\scalebox{0.84}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{\textbf{Methods}} &
    \multirow{2}{*}{\textbf{Type}} &
    \multicolumn{4}{c|}{\textbf{Motion Coder}} &
    \multicolumn{3}{c|}{\textbf{Residual Coder}} &
    \multicolumn{3}{c|}{\textbf{Entropy Coding}} \\
    \cline{3-12}
    \multirow{1}{*}{} &
    \multirow{1}{*}{} &
    \multicolumn{1}{c|}{\textbf{No cond.}} &
    \multicolumn{1}{c|}{\textbf{Residual}} &
    \multicolumn{1}{c|}{\textbf{RNN}} &
    \multicolumn{1}{c|}{\textbf{Cond.}} &
    \multicolumn{1}{c|}{\textbf{Residual}} &
    \multicolumn{1}{c|}{\textbf{RNN}} &
    \multicolumn{1}{c|}{\textbf{Cond.}} &
    \multicolumn{1}{c|}{\textbf{Hyperprior}} &
    \multicolumn{1}{c|}{\textbf{Temporal}} &
    \multicolumn{1}{c|}{\textbf{Spatial}}\\
    
    
    \hline
    DVC\cite{lu2019dvc} & VAE & $\surd$ & & & & $\surd$ & & & & & \\
    \hline
    MLVC\cite{lin2020m} & VAE & & $\surd$ && & $\surd$ & & & & & \\
    \hline
    SSF\cite{agustsson2020scale} & VAE & $\surd$ & && & $\surd$ & & & $\surd$ & $\surd$ & \\
    \hline
    NVC\cite{liu2020neural} & VAE & $\surd$ && & & $\surd$ & & & $\surd$ & $\surd$ & $\surd$ \\
    \hline
    RLVC\cite{yang2020learning} & VAE & & & $\surd$ & & & $\surd$ & & $\surd$ & $\surd$ & \\
    \hline
    ACCV'20\cite{golinski2020feedback} & VAE & & & $\surd$ & & & $\surd$ & & & & \\
    \hline
    RaFC\cite{hu2020improving} & VAE & $\surd$ & & & & $\surd$ & & & $\surd$ & & $\surd$ \\
    \hline
    MMSP'20\cite{ladune2020optical} & VAE & $\surd$ & & & & & & $\surd$ & $\surd$ & & \\
    \hline
    DCVC\cite{li2021deep} & VAE & $\surd$ & & & & & & $\surd$ & $\surd$ & $\surd$ & $\surd$ \\
    \hline
    Ours & ANF & & & & $\surd$ & & & $\surd$ & $\surd$ & $\surd$ & \\
    \hline
    \end{tabular}
}
}
\end{table*}

==> chapter/5-2_table_motion.tex <==

% \vspace{-1.5em}
% \begin{table}[]
%     \centering
%     \caption{Comparison of conditional motion coding, predictive motion coding, and intra motion coding. The last row is our proposed method.}
%     \label{tab:study_motion}
%     \tabcolsep=12pt
%     \resizebox{0.63\linewidth}{!}{
%         \begin{tabular}{cccc}
%             \toprule
%             Input of Motion Coder   & Condition       & BD-Rate     \\ \hline
%             $f_t$                   & -               &    -33.4\%  \\
%             $f_t - f_c$             & -               &    -35.3\%  \\
%             $f_t$                   &$\hat{f}_{t-1}$  &    -35.2\%  \\ 
%             $f_t$                   &$f_c$            &    -42.5\%  \\
%             \bottomrule
%         \end{tabular}
%     }
% \vspace{-1.5em}
% \end{table}

==> chapter/5-3_table_layer.tex <==

% %\vspace{-0.3em}
% \begin{table}[]
%     \centering
%     \caption{Comparison of the conditional motion and inter-frame coders with a varied number of autoencoding transforms. The last row is our proposed method, and CANF stands for conditional ANF.}
%     \vspace{-0.2em}
%     \label{tab:study_layer}
%     \tabcolsep=12pt
%     \resizebox{0.63\linewidth}{!}{
%         \begin{tabular}{cccc}
%             \toprule
%             Motion Coder                      & Inter-frame Coder & BD-Rate  \\ \hline
%             DVC~\cite{dvclu} & 1-step CANF       & -31.4\%      \\
%             DVC~\cite{dvclu} & 2-step CANF       & -31.9\%      \\ \hline\hline
%             1-step CANF                       & 2-step CANF       & -38.1\%      \\
%             2-step CANF                       & 2-step CANF       & -42.5\%      \\
%             \bottomrule
%         \end{tabular}
%     }
% \vspace{-0.8em}
% \end{table}
